A Reinforcement Learning Approach to Sensing Design in Resource-Constrained Wireless Networked Control Systems

In this paper, we consider a wireless network of smart sensors (agents) that monitor a dynamical process and send measurements to a base station that performs global monitoring and decision-making. Smart sensors are equipped with both sensing and computation, and can either send raw measurements or process them prior to transmission. Constrained agent resources raise a fundamental latency-accuracy trade-off. On the one hand, raw measurements are inaccurate but fast to produce. On the other hand, data processing on resource-constrained platforms generates accurate measurements at the cost of non-negligible computation latency. Further, if processed data are also compressed, latency caused by wireless communication might be higher for raw measurements. Hence, it is challenging to decide when and where sensors in the network should transmit raw measurements or leverage time-consuming local processing. To tackle this design problem, we propose a Reinforcement Learning approach to learn an efficient policy that dynamically decides when measurements are to be processed at each sensor. Effectiveness of our proposed approach is validated through a numerical simulation with case study on smart sensing motivated by the Internet of Drones.

==> Sections/homogeneous-sensors-old.tex <==
%!TEX_root = ../processing_networks_estimation_RL.tex

\subsubsection{Homogeneous Sensors}\label{sec:hom-sens}

In this case, all sensors have identical sensing modes and noise statistics,
\begin{equation}\label{eq:hom-sensors}
    \yi{k}{i} = \x{k} + \vi{k}{i}, \qquad \vi{k}{i}\sim\gauss(0,\V{k}),
\end{equation}
with %$C\in\Real{m\times n}$ and
$ \V{k} = \varRaw $ or $ \V{k} = \varProc $ for raw and processed data, respectively.
Further, all sensors have computational delays $ \delayRaw $ and $ \delayProc $,
and communication delays $ \delayCommRaw $ and $ \delayCommProc $
($ \delayComm $ in case of no compression),
for raw and processed data, respectively.
Such \textit{homogeneous sensor} scenario
models the special but relevant case where sensors are interchangeable.
This happens, \eg with sensors monitoring
temperature in large plants or %concentrations in chemical plants, %, to name a few.
with smart cameras extracting high-level information
such as object pose. % or room occupancy. % position of a vehicle. % or occupancy in a room. % or another robot.

\subsubsection{Problem Simplification}
In this scenario, %data processing is not tied to specific sensors,
%rather than deciding on local processing \textit{at each sensor}
one just needs to decide \textit{how many}, rather than \emph{which}, sensors shall process at each time.
Hence, the amount of sensing configurations drops to $ N+1 $,
%\ie grow linearly with the number of sensors,
%yielding a tractable search space.% % for the sensing policies.
greatly reducing the search space.%
\footnote{In the general case with $ C $ processing settings for each sensor, the total amount of configurations becomes $\binom{N+C-1}{C-1}$.}
Accordingly,
we shift attention to %from individual sensor policies to %making from decentralized (individual sensors)
%to centralized, namely, the base station generates a 
a centralized \emph{\homProcPol}.
%and broadcast processing decisions to all sensors in the network.
%\LB{Forse dovremmo rinominare le processing policies per i singoli sensori del tipo \textit{sensor processing policy}}

\begin{definition}[Homogeneous sensing policy] \label{def:hom_case}
	A \emph{\homProcPol} is a sequence $ \policyHom = \{\decisionHom{\ell}\}_{\ell=1}^L $,
	where each \emph{homogeneous decision} $ \decisionHom{\ell} \in \{0,\dots,N\} $ is taken at time $ \kell[]{} $.
	If $ \decisionHom{\ell} = p $, then $ p $ sensors process their measurements
%	encodes how many sensors will process
	and $ N-p $ send them raw between times $ \kell[]{} $ and $ \kell[+1]{} $.
	Without loss of generality, we set $ k^{(1)} = k_0 $ and $ \kL < K $.
\end{definition}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{Images/delayed-meas-centr}
	\caption{Homogeneous sensors ruled by policy $ \policyHom $.
	    As decision $ \decisionHom{\ell} $ is communicated, % at time  $ \kell{} $,
	    the $ i $th sensor disregards current measurement (red cross) and
	    immediately switches to raw mode, acquiring a new sample.
    }
	\label{fig:delayed-meas-centr}
\end{figure}

In words, the base station decides for all sensors at predefined time instants, % and communicates such decisions.
which is convenient both in practical applications
%This entails additional design flexibility
and to set up our learning procedure. %our learning framework.
However, frequency of decisions may be arbitrary, in general.
%(up to consistency with delays).

Centralized decisions may be communicated while some sensors
are still processing their data. %, so that they cannot transmit them and switch mode immediately.
%because of processing delays. % without discarding acquired data.
%The following assumption imposes that gathered information be not "wasted".
%This new sensing dynamics is depicted in~\autoref{fig:delayed-meas-centr}.
According to standard real-time control~\cite{5510096,s22041638,8950356},
we assume what follows.

\begin{ass}[Sampling frequency with \homProcPol]\label{ass:decision-time-centralized-policy}
	Decision $ \decisionHom{\ell} $ affects the minimum amount of sensors possible.
	When a sensor is commanded to switch mode,
	the current measurement is immediately discarded
	and sampling restarts with the new mode.
	Hence, given a measurement sampled at time $ k $,
	dynamics~\eqref{eq:sensor-frequency} becomes
	\begin{equation}\label{eq:sensor-frequency-centralized-policy}
	s_i^h(k) \doteq \begin{cases}
		\min\left\lbrace k + \delayRaw,\kell{}\right\rbrace  & \text{if }\yi{k}{i} \text{ raw}\\
		\min\left\lbrace k + \delayProc,\kell{}\right\rbrace & \text{if }\yi{k}{i} \text{ processed},\\
	\end{cases}
    \end{equation}
    where $ \yi{k}{i} $ is sampled before decision $ \decisionHom{\ell} $ is communicated,
    and it is discarded if it is not transmitted by time $ \kell{} $.
    Further, we require $ \kell[+1]{} \ge \kell{} + \delayProc, \ell = 1,\dots,L-1 $.
%	complete ongoing processing, %processed according to $ \decisionHom{\ell-1} $,
%	send processed measurements to the base station, and then start transmitting raw data. % immediately after its transmission.
\end{ass}

\iffalse
%This leads to the following definition.
%\LB{Da capire se questa ipotesi è sensata anche con sensori eterogenei,
%o se dovremmo lasciarli switchare in modo asincrono con $ \kell_i $ (non so se sia fattibile RL-wise)}
\begin{ass}[Homogeneous policy measurements]\label{ass:measurements-decision-ell}
%	Decision $ \decision{\ell}{i} $ is taken at time $ \kell{i} \in [k_0,K] $.
%	If $ \decision{\ell}{i} \in \{\mathrm{r},\mathrm{p}\}$,
	Under decision $ \decisionHom{\ell} $, the $ i $th sensor acquires measurements
	%	processes according to $ \decision{\ell}{i} $
	at times
	\begin{gather}\label{eq:decision-timestamps}
		\decisionTimestamps{\ell}{i} \doteq \left\lbrace\kell{}, \kell{i} + \decisionDelay{\ell},\dots, \kell[+1]{i} - \decisionDelay{\ell}\right\rbrace,
		\ 0 < \ell < L,\\
		\decisionTimestamps{L}{i} \doteq \left\lbrace\kL[i],\dots, K - \mathrm{mod}\left(K-\kL[i],\decisionDelay{L}\right)\right\rbrace.
	\end{gather}
	%	where $  \decisionDelay{\ell}{i} = \delayRaw{i} $ if $ \decision{\ell}{i} = \mathrm{r} $ 
	%	and $ \decisionDelay{\ell}{i} = \delayProc{i} $ if $ \decision{\ell}{i} = \mathrm{p} $.
	%	and such measurements are raw or processed according to decision $ \decision{\ell}{i} $.
%	The first decision is alway taken at the first time instant, $ k_i^{(0)} = k_0 $,
%	and $ K \ge \kL[i]$ is the maximum time associated with $ \policy[i] $.
%	W.l.o.g., we require $ \lvert\decisionTimestamps{\ell}{i}\rvert \ge 1 $ for all $ i\in\sensSet, \ \ell = 1,\dots,L $.
\end{ass}

\begin{definition}[Available sensory data]\label{def:data-collected}
	According to Assumptions~\ref{ass:delays-variances} and~\ref{ass:measurements-decision-ell},
	all measurements from $ i $th sensor available at the base station at time $ k $ are
	\begin{gather}\label{eq:sequence-measurements}
		\measurements{k}{i} \doteq \left\lbrace \yi{h}{i} : h\in\bigcup_{\ell=1}^L \decisionTimestamps{\ell}{i}, \; h \le k - \delayRec{h} \right \rbrace.
%		\timestamps{k}{i} \doteq \bigcup_{\ell} \decisionTimestamps{\ell}{i}.
	\end{gather}
\end{definition}
%	where the total sequence of timestamps is
%	 $ \timestamps{k}{i} $ depends on the processing policy $ \policy[i] $
%	and is defined as
%	\begin{equation}\label{eq:sequence-timestamps}
%		\timestamps{k}{i}\left(\policy[i]\right) \doteq \bigcup_{\ell=1}^L \decisionTimestamps{\ell}{i}.
%	\timestamps{k}{i}\left(\policy[i]\right) \doteq \left\lbrace k_0, k_0 + \decisionDelay{1}{i},\dots,k_L,\dots, k - \mathrm{mod}\left(k-k_L,\decisionDelay{L}{i}\right) \right\rbrace.
%	\end{equation}
In words, %given current time $ k $,
$ \timestamps{k}{i}\left(\policy[i]\right) $ gathers all acquisition times induced by $ \policy[i] $
such that their associated measurements
are available at the base station at time $ k $.
In particular, %\emph{acquired} before $ k $ but \emph{transmitted} after $ k $
some data \emph{acquired} before time $ k $
are not %yet available and not
included in $ \measurements{k}{i}\left(\policy[i]\right) $
because of their computational delays.
Note that $ \measurements{K}{i}(\policy[i]) $ gathers all data collected under $ \policy[i] $
available at time $ K $.
%	before $ k $
%	when $ i $th sensor sampled the state
%	when $ i $th sensor acquired data according to $ \policy[i] $
%	and sent them to the base station.
In the following,
%	with a slight abuse of notation,
we occasionally drop the argument %and write $ \measurements{k}{i}, \timestamps{k}{i} $ 
for the sake of readability.
\fi

\begin{comment}
~\cref{ass:decision-time-centralized-policy}
affects the nominal sampling frequency~\eqref{eq:sensor-frequency} of switched sensor $ i $ as
\begin{equation}\label{eq:sensor-frequency-centralized-policy}
	s_i^h(k) \doteq \begin{cases}
		\min\{k + \delayRaw,\kell{}\}  & \text{if }\yi{k}{i} \text{ raw},\\
		\min\{k + \delayProc,\kell{}\} & \text{if }\yi{k}{i} \text{ processed},\\
	\end{cases}
\end{equation}
where $ \yi{k}{i} $ is collected before decision $ \decisionHom{\ell} $ is communicated. % at time $ \kell{} $.
%does not affect sampling dynamics~\eqref{eq:sensor-frequency}.
\end{comment}
In view of~\cref{ass:decision-time-centralized-policy},
the available sensory data at the base station %at time $ k $
now exclude
measurements discarded by overlapping decisions. %~\eqref{eq:sensor-frequency-centralized-policy}. % and~\cref{ass:decision-time-centralized-policy}.
Formally, for the $ i $th sensor, such data
are raw (resp., processed) measurements $ \yi{k}{i} $ sampled under decision $ \decisionHom{\ell-1} $
such that $ k + \delayRaw > \kell{} $ (resp., $ k + \delayProc > \kell{} $),
\ie their generation ends after a \textit{different} mode is imposed at time $ \kell{} $ by decision $ \decisionHom{\ell} $.
Figure~\ref{fig:delayed-meas-centr} illustrates the new sampling dynamics, with the second measurement of the $ i $th sensor discarded at time $ \kell{} $.
To avoid excessive notational burden, we simply write $ \measurements[\policyHom]{k} $
to denote available data at the base station at time $ k $ according to~\eqref{eq:sensor-frequency-centralized-policy} and
the discussed data dropping mechanism imposed by policy $ \policyHom $,
that prunes some measurements from the set $ \measurements[]{k} $.

In this scenario, \cref{prob:optimal-estimation} simplifies as follows.

\begin{prob}[Sensing Design for Homogeneous Processing Network]\label{prob:optimal-estimation-hom}
    Given system~\eqref{eq:stateEquation},~\eqref{eq:hom-sensors} with Assumptions~\ref{ass:delays-variances}--\ref{ass:decision-time-centralized-policy}
    and sequence $ \{\kell{}\}_{\ell=1}^L $, $ \kell[+1]{} \ge \kell{} + \delayProc \,\forall\ell<L$, $ L < K $,
    find the optimal \homProcPol $ \policyHom $,
    with $ \ell $th decision $ \decisionHom{\ell} $ scheduled at time $ \kell{} $,
	so as to minimize the time-averaged estimation error variance with horizon $K$,
    \begin{equation}\label{eq:prob-optimal-estimation-hom}
    	\begin{aligned}
	        \argmin_{\policyHom\in\Pi_\text{hom}}& &&\frac{1}{K}\sum_{k=k_0}^K \tr{\Pmat{k}{\policyHom}}\\
			\text{s.t.}& &&\Pmat{k}{\policyHom} = \kalman{\measurements[\policyHom]{k}}\\
			& &&\Pmat{k_0}{\policyHom} = P_0,
    	\end{aligned}
    \end{equation}
	where the Kalman predictor $ \kalman{\cdot} $ computes at time $ k $ state estimate $ \xhat{k}{\policyHom} $ and error covariance matrix $ \Pmat{k}{\policyHom} $
	using data $ \measurements[\policyHom]{k} $ available at the base station according to $ \policyHom $,
	and $ \Pi_\text{hom} $ gathers all causal homogeneous sensing policies.
\end{prob}

\begin{rem}[Heterogeneous sensors]\label{rem:het-sens}
	\cref{prob:optimal-estimation-hom} can be easily generalized to heterogeneous sensors,
	whereby decisions are centralized and the base station schedules \emph{which} sensors process their data
	at each decision $ \policy[\ell] $. %for each time interval $ \left(\kell{},\kell[+1]{\ell}\right) $.
	However, while the centralized implementation reduces complexity associated with optimizing asynchronous mode switching of agents,
	the space of sensing configurations may still explode with the amount of sensors.
	In order to keep computational burden of learning reasonable,
	we focus on the homogeneous case in the following, %throughout the rest of this paper,
	with the understanding that the heterogeneous case
	increases computational complexity but can be embedded into our problem formulation and learning framework with little effort.
	Future work will focus on enabling compute-efficient strategies for (large-scale) heterogeneous networks,
	possibly with distributed methods such as multi-agent reinforcement learning,
	but this is out of the scope of this paper.
%	\red{Mention that we can also deal with heterogeneous sensors?}
\end{rem}
